A Polynomial-time Algorithm for Outerplanar Diameter Improvement

The Outerplanar Diameter Improvement problem asks, given a graph $G$ and an integer $D$, whether it is possible to add edges to $G$ in a way that the resulting graph is outerplanar and has diameter at most $D$. We provide a dynamic programming algorithm that solves this problem in polynomial time. Outerplanar Diameter Improvement demonstrates several structural analogues to the celebrated and challenging Planar Diameter Improvement problem, where the resulting graph should, instead, be planar. The complexity status of this latter problem is open.

==> conclusions.tex <==
\section{Conclusions and further research}
\label{sec:conclusions}

\ign{TO DO!!}\\

\noindent \ign{This is just some disjoint stuff from previous versions:}

Can we get an exhaustive list of forbidden subgraphs?

 its \textsc{Yes}-instances are closed under taking of
minors\footnote{To see this, \ign{FINISH!!}} which, according to the meta-algorithmic consequence of the Graph Minors series of Robertson and Seymour~\cite{RobertsonS95-XIII,RobertsonS04-XX}, implies that \PDIfull is in {\sf FPT}.


\begin{hey}{Problem}
  How efficiently can a graph be completed by addition of edges into an outerplanar graph of minimum diameter ?
\end{hey}





